Millimeter and Submillimeter Excess Emission in M33 revealed by Planck and LABOCA

Previous studies have shown the existence of an excess of emission at submillimeter (submm) and millimeter (mm) wavelengths in the spectral energy distribution (SED) of many low-metallicity galaxies. The goal of the present study is to model separately the emission from the star forming (SF) component and the emission from the diffuse interstellar medium (ISM) in the nearby spiral galaxy M33. We decomposed the observed SED of M33 into its SF and diffuse components. Mid-infrared (MIR) and far-infrared (FIR) fluxes were extracted from Spitzer and Herschel data. At submm and mm wavelengths, we used ground-based observations from APEX to measure the emission from the SF component and data from the Planck space telescope to estimate the diffuse emission. Both components were separately fitted using radiation transfer models based on standard dust properties and a realistic geometry. Both modeled SEDs were combined to build the global SED of M33. In addition, the radiation field necessary to power the dust emission in our modeling was compared with observations from GALEX, Sloan, and Spitzer. Our modeling is able to reproduce the observations at MIR and FIR wavelengths, but we found a strong excess of emission at submm and mm wavelengths, where the model expectations severely underestimate the LABOCA and Planck fluxes. We also found that the ultraviolet (UV) radiation escaping the galaxy is 70% higher than the model predictions. We determined a gas-to-dust mass ratio Gdust~100, significantly lower than the value expected from the sub-solar metallicity of M33. We discussed different hypotheses to explain the discrepancies found in our study (i.e., excess of emission at submm and mm wavelengths, deficit of UV attenuation, and abnormally low value of Gdust), concluding that different dust properties in M33 is the most plausible explanation.

==> 00_CONFIG/Astro/Observations.tex <==
%
% Template table for the observations
% Author: Israel Hermelo
% Created: 2015.APR.01
% Last update: 2016.JAN.27
%
%
%

\begin{table*}[!htbp]
\centering
\vspace{26pt}
\begin{tabular}{l c c c c c l l} \hline \noalign{\medskip}
%
\textnormal{Telescope}               &  % Column 1
\textnormal{Instrument}              &  % Column 2
$\lambda_{\rm 0}$                    &  % Column 3
$\nu_{\rm 0}$                        &  % Column 4
\textnormal{FWHM}                    &  % Column 5
$\Delta_{\rm CAL}$                   &  % Column 6
\textnormal{Band name}               &  % Column 7
\textnormal{References}              \\ % Column 8
%
\textnormal{}                        &  % Column 1
\textnormal{or filter}               &  % Column 2
\microns{}                           &  % Column 3
\GHz{}                               &  % Column 4
\textnormal{}                        &  % Column 5
\%                                   &  % Column 6
\textnormal{}                        &  % Column 7
\textnormal{}                           % Column 8
\\\noalign{\smallskip} \hline \noalign{\medskip}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\noalign{\smallskip}
%
\GALEX{}      & FUV                 &   0.154 & 1\,946\,704 &  \arcseconds{4}{2}    & 10 & \GALEX{FUV}                 & {\cite{}}                       \\\noalign{\smallskip}
              & NUV                 &   0.232 & 1\,292\,209 &  \arcseconds{5}{3}    & 10 & \GALEX{NUV}                 & {\cite{}}                       \\\noalign{\smallskip}\hline \noalign{\medskip}
%
%
\SLOAN{}      & u                   &   0.355 &     12\,650 &                       &  2  & \SLOAN{u}                  & {\cite{}}                       \\\noalign{\smallskip}
              & g                   &   0.469 &    844\,486 &                       &  1  & \SLOAN{g}                  & {\cite{}}                       \\\noalign{\smallskip}
              & r                   &   0.617 &    485\,887 & \arcseconds{1}{4}     &  1  & \SLOAN{r}                  & {\cite{}}                       \\\noalign{\smallskip}
              & i                   &   0.748 &    400\,792 &                       &  1  & \SLOAN{i}                  & {\cite{}}                       \\\noalign{\smallskip}
              & z                   &   0.893 &    335\,714 &                       &  1  & \SLOAN{z}                  & {\cite{}}                       \\\noalign{\smallskip}\hline \noalign{\medskip}
%
%
KPNO          & \Halpha             &   0.657 &    456\,305 & \arcseconds{6}{6}     & 15  & \Halpha                    & {\cite{}}                       \\\noalign{\smallskip}\hline \noalign{\medskip}
%
%
\SPITZER{}    & \CAMERAmu{IRAC}{}   &    3.55 &     84\,449 & \arcseconds{2}{5}     &  5  & \CAMERAmu{IRAC}{3.6}       & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAmu{IRAC}{}   &    4.49 &     66\,769 & \arcseconds{2}{9}     &  5  & \CAMERAmu{IRAC}{4.5}       & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAmu{MIPS}{}   &    23.7 &     12\,650 & \arcseconds{6}{3}     &  4  & \CAMERAmu{MIPS}{24}        & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAmu{MIPS}{}   &    71.4 &      4\,199 & \arcseconds{16}{}     &  7  & \CAMERAmu{MIPS}{70}        & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAmu{MIPS}{}   &     156 &      1\,923 & \arcseconds{40}{}     & 12  & \CAMERAmu{MIPS}{160}       & {\cite{}}                       \\\noalign{\smallskip}\hline \noalign{\medskip}
%
%
\HERSCHEL{}   & \CAMERAmu{PACS}{}   &    70.0 &      4\,283 & \arcseconds{5}{6}     & 10  & \CAMERAmu{PACS}{70}        & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAmu{PACS}{}   &     100 &      2\,998 & \arcseconds{9}{8}     & 10  & \CAMERAmu{PACS}{100}       & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAmu{PACS}{}   &     160 &      1\,874 & \arcseconds{13}{6}    & 20  & \CAMERAmu{PACS}{160}       & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAmu{SPIRE}{}  &     250 &      1\,199 & \arcseconds{18}{1}    & 10  & \CAMERAmu{SPIRE}{250}      & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAmu{SPIRE}{}  &     363 &         826 & \arcseconds{24}{9}    & 10  & \CAMERAmu{SPIRE}{350}      & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAmu{SPIRE}{}  &     517 &         580 & \arcseconds{36}{4}    & 10  & \CAMERAmu{SPIRE}{500}      & {\cite{}}                       \\\noalign{\smallskip}\hline \noalign{\medskip}
%
%
\APEX{}       & \CAMERAmu{LABOCA}{} &     870 &         345 & \arcseconds{19}{2}    & 10  & \CAMERAmu{LABOCA}{870}     & {\cite{}}                       \\\noalign{\smallskip}\hline \noalign{\medskip}
%
%
\PLANCK{}     & \CAMERAghz{HFI}{}   &     350 &         857 & \arcminutes{4}{63}    & 10  & \CAMERAmu{HFI}{350}        & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAghz{HFI}{}   &     550 &         545 & \arcminutes{4}{84}    & 10  & \CAMERAmu{HFI}{550}        & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAghz{HFI}{}   &     850 &         353 & \arcminutes{4}{86}    &  3  & \CAMERAmu{HFI}{850}        & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAghz{HFI}{}   &  1\,380 &         217 & \arcminutes{5}{01}    &  3  & \CAMERAmm{HFI}{1.4}        & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAghz{HFI}{}   &  2\,096 &         143 & \arcminutes{7}{27}    &  3  & \CAMERAmm{HFI}{2.1}        & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAghz{HFI}{}   &  3\,000 &         100 & \arcminutes{9}{66}    &  3  & \CAMERAmm{HFI}{3.0}        & {\cite{}}                       \\\noalign{\smallskip}
              & \CAMERAghz{LFI}{}   & 10\,000 &          30 & \arcminutes{32}{3}    &  3  & \CAMERAmm{LFI}{10}         & {\cite{}}                       \\\noalign{\smallskip}\hline \noalign{\medskip}
%
%
\EFFELSBERG{} & \CAMERAmm{S}{36}    & 35\,903 &        8.35 & \arcminutes{1}{39}    &  *  & \CAMERAmm{S}{36}           & {\cite{}}                       \\\noalign{\smallskip}\hline \noalign{\medskip}
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\caption{%
Summary of the observations used in this study.
\label{tab:observations}}
\end{table*}
%
%
% GALEX: http://iopscience.iop.org/0067-0049/173/2/682/fulltext/
% SLOAN: http://iopscience.iop.org/0004-637X/674/2/1217/
% MIPS160: http://www.jstor.org/stable/10.1086/521880
%
% PACS: http://herschel.esac.esa.int/Docs/PACS/html/ch03.html#sec-characteristics-photometer
% SPIRE: http://herschel.esac.esa.int/twiki/bin/view/Public/SpireCalibrationWeb#SPIRE_calibration_and_performanc
% LFI: http://wiki.cosmos.esa.int/planckpla/index.php/Beams_LFI
%


==> 00_CONFIG/Layout/Personal.tex <==
%
% Author         Israel Hermelo
% Description    LaTeX file with personal info
% Last update    2015.NOV.03
%
%
\newcommand{\name}        {Dr. Israel Hermelo}
\newcommand{\birth}       {February 1, 1983 (Spain)}
\newcommand{\institution} {Institut de Radioastronomie Millimétrique}
\newcommand{\group}       {Astronomy \& Science Support Group}
\newcommand{\position}    {IRAM 30\,m single-dish radiotelescope}
\newcommand{\street}      {Avenida Divina Pastora, 7}
\newcommand{\city}        {18012, Granada (Spain)}
\newcommand{\email}       {hermelo@iram.es}
\newcommand{\workphone}   {+34~958\,80\,54\,77}
\newcommand{\cellphone}   {+34~647\,93\,12\,90}
\newcommand{\photo}       {../../Database/Personal/hermelo2014lowres.png}
%
\newcommand{\signature}   {\hspace{270pt}Yours faithfully,
                           %
                           \begin{figure}[!ht]%
                             \hspace{250pt}\includegraphics[width=0.35\textwidth]{../../Database/Personal/signature.png}%
                           \end{figure}
                           %
                           \par\vspace{0pt}
                           %
                           \hspace{255pt} Dr. Israel Hermelo%
                           %
                           \par\vspace{4pt}
                           %
                           \hspace{255pt} \today%
                          }
%
%


==> 03_PHOTOMETRY/PhotometryCAT.tex <==
% The SED of M33
% Photometry
% Last update: 2015.JAN.12
%
%
\section{Photometry \label{sec:Photometry}}
%
Prior to performing the photometry, we first homogenized all the images
to the same data unit in order to measure all fluxes in \Jy{}/pixel
(with a pixel size of \arcseconds{14}{}).
%
\comment{%
%
Bright foreground stars were removed from the UV and optical data.
%
}
%
We then convolved all the data to the resolution of \CAMERAmu{SPIRE}{500} using the set of
kernels provided by \citet[][]{2011PASP..123.1218A}%
%
\footnote{http://www.astro.princeton.edu/~ganiano/Kernels.html},
%
with the only exception of \PLANCK{} data, which have a coarser resolution than the
\CAMERAmu{SPIRE}{500} image, and therefore, they were only used to obtain the total
photometry of \MESSIER{33}.
%
Using the IRAF task \WREGISTER, we then regridded all the images
to the pixel size of the \CAMERAmu{SPIRE}{500} map.
%
In this section we describe how we extracted the photometry of the different components,
how we corrected our measurements from undesired contributions
(e.g., \CO{}{} line emission),
and how the errors were handled.
%
Color corrections were applied to all the MIR/FIR/submm/mm fluxes
(see \App{app:CC} for details)
%
%
\subsection{Total stellar and dust emission \label{subsec:total}}
%
The total emission of \MESSIER{33} was measured using an aperture for the
entire galaxy defined by a radius of \arcminutes{35}{} (\kpc{8.5})
and an inclination of \degrees{57}.
%
This aperture is slightly larger than the one used by
\citet[][]{2010A&A...518L..67K}
in order to enclose the whole emission of the \PLANCK{} bands,
which have a much poorer resolution than the data used by these authors.
%
The flux densities measured for the total stellar and total dust emission
are listed \Tab{tab:M33_Photometry}.
%
\input{97_IDL/TABLES/M33_Photometry}
%
%
\subsection{Emission from the SF component \label{subsec:SF}}
%
\comment{%
%
The first step to to extract the emission from the SF component
was building a complete catalog of SF regions.
%
Based on the the smoothed version of the \Halpha\ image we carefully selected
a total of 358 regions (see the top panel of \Fig{fig:M33components}).
%
Rather than circles we decided to use ellipses with the aim of obtaining
the best match possible to the irregular shape of the SF regions.
%
}
%

%
\comment{%
%
Then, for each one of these 358 ellipses, we measure the median value within
a narrow annulus, which we assumed to be a reliable estimate of the diffuse
emission in the background/foreground along the line-of-sight of the SF region.
%
All the pixels within the ellipse where substituted by this median value,
thus obtaining a full map of the diffuse emission of \MESSIER{33}
(see the bottom panel of \Fig{fig:M33components}).
%
We repeated the process for all the bands available with the exception of
\PLANCK{} data because of their lower spatial resolution.
%
}
%

%
\comment{%
%
Finally, for each band we subtracted the diffuse emission map from the total
emission to obtain a map that only includes emission from the SF component.
%
From this map it is straightforward to extract the photometric values of
the SF component, which are shown in \Tab{tab:M33_Photometry}.
%
}
%

%
%
%
\ImageCol{0.48}
         {./98_FIGURES/M33comp_Halpha.png}
         {fig:M33components}
         {%
          \comment{%
          %
          \Halpha\ emission of \MESSIER{33} smoothed to the resolution of the
          \CAMERAmu{SPIRE}{500} band.
          %
          The top panel shows the total emission while the bottom panel corresponds to our
          estimate of the diffuse emission.
          %
          The apertures used to build the map of the diffuse emission are shown as red dashed ellipses.
          %
          The diffuse emission represents \percent{70} of the total \Halpha\ emission.
          %
          Both images share the same scale and contrast represented by the colorbar at the bottom.
          %
          }
          %
          }
%
%
%
\subsection{Diffuse emission \label{subsec:diffuse}}
%
\comment{%
%
The photometry of the diffuse component
(see \Tab{tab:M33_Photometry})
was calculated as the difference between our
measurements of the total emission
(see \Sec{subsec:total})
and the emission from the SF component
(see \Sec{subsec:SF}).
%
}
%
In those cases where the angular resolution did not allow to extract
the emission from the SF regions
(i.e., \PLANCK{} data),
the diffuse emission was estimated by subtracting the flux of the SF component
predicted by the model of \citet[][]{2008ApJS..176..438G}
from the total flux of \MESSIER{33}.
%

%
Even though our estimates of the diffuse emission
are well constrained by this method in most wavelengths,
the lack of data points constraining the SED of the SF component
between \CAMERAmu{LABOCA}{870}
and the free-free emission at \cm{3.6} from \citet[][]{2007A&A...475..133T}
introduces some uncertainties.
%
As a cautionary measure, we  do not include the indirect
data points in the fitting procedure.
%
% However, it is noteworthy that observations
% of the brightest SF region of \MESSIER{33}, \NGC{604},
% with the Goddard-IRAM Superconducting \mm{2} Observer (GISMO)
% at the IRAM~\meters{30} telescope show no deviations from the value expected
% based on an extrapolation with the \citet[][]{2008ApJS..176..438G}
% model in this range (Rela\~no et al., in prep.).
%
%
%
%
%
\subsection{CO contamination \label{sec:CO}}
%
The emission from the \CO{}{} rotational transitions
\CO{1}{0} at \mm{2.6} (\GHz{115}),
\CO{2}{1} at \mm{1.3} (\GHz{230}), and
\CO{3}{2} at \microns{870} (\GHz{345}),
fall into the bandpasses of the
\PLANCK{} \mm{3.0}, \mm{1.4}, and \microns{850} filters,
respectively \citep[][]{2014A&A...571A..13P}.
%
In addition, the \CAMERAmu{LABOCA}{870} filter is also affected
by the \CO{3}{2} line.
%

%
In order to correct the measured continuum fluxes for the contribution
of these major gas cooling lines,
we made use of \CO{2}{1} observations
\citep[][]{2014A&A...567A.118D}
obtained with the HEterodyne Receiver Array
\citep[HERA, ][]{2004A&A...423.1171S}
mounted on the IRAM~\meters{30} telescope on Pico Veleta (Spain).
%

%
\citet[][]{2014A&A...567A.118D} mapped the inner \kpc{\sim7} of \MESSIER{33}
with an angular resolution of \arcseconds{12}{}.
%
These authors reported a total \CO{2}{1} luminosity of
$2.8\times10^7\,\Kelvin{}\,\kms{}\,pc{}^2$,
which corresponds to a flux of \Sco{}{}{6.5\times10^4}.
%
For the \CAMERAmm{PLANCK}{1.4} filter,
which has a width of \GHz{64.5} (\kms{87\,433})
and a transmission close to \percent{100} at the frequency of the \CO{2}{1}
line \citep[see \Fig{}~1 in][]{2014A&A...571A..13P},
we measured a flux density of \Jy{17.4}.
%
Using these values we estimate that \percent{4.3}
of the flux density of \MESSIER{33} measured with this filter
comes from \CO{2}{1} line emission.
%

%
The \CO{1}{0} line emission was also observed with the
IRAM \meters{30} telescope in a radial cut along the major axis of \MESSIER{33}
\citep[][]{2010A&A...520A.107B}.
%
Comparing these data with their map, \citet[][]{2014A&A...567A.118D}
found a constant ratio $I_{\CO{1}{0}}/I_{\CO{2}{1}}$ of 1.25
in the overlapping area.
%
Assuming that this ratio can be extrapolated to the whole disk of \MESSIER{33},
we could estimate the flux of \CO{1}{0} as:
%
\begin{equation}
\label{eq:Sco10}
\Sco{1}{0}{} = 1.25 \,\times\, \left( \frac{115}{230} \right)^2 \Sco{2}{1}{} = \Sco{}{}{2.0\times10^4}.
\end{equation}
%
We measured a flux density of \Jy{1.56}
with the \CAMERAmm{PLANCK}{3.0} filter,
which has a width of \GHz{32.9} (\kms{97\,762})  and
a transmission of about \percent{60} at the frequency of the line.
%
Therefore, we estimate that the \CO{1}{0} emission is responsible for
\percent{7.9} of the flux measured with the \CAMERAmm{PLANCK}{3.0} band.
%

%
Finally, the contamination due to the emission from the \CO{3}{2} line
was estimated assuming a ratio $I_{\CO{3}{2}}/I_{\CO{2}{1}}\sim1$,
i.e.:
%
\begin{equation}
\label{eq:Sco32}
\Sco{3}{2}{} \sim \left( \frac{345}{230} \right)^2 \Sco{2}{1}{} = \Sco{}{}{14.6\times10^4}.
\end{equation}
%
With the \CAMERAmu{PLANCK}{850} filter we measured
a flux density of \Jy{74.3}.
%
Using a width of \GHz{101.4} (\kms{85\,032})
and a transmission \percent{\sim100},
we found that the contribution from the \CO{3}{2} line
to the \CAMERAmu{PLANCK}{850} is \percent{\sim2.3}.
%
In the case of the \CAMERAmu{LABOCA}{870} filter,
we measured a flux density of \Jy{37.1}.
%
For a width of \GHz{59.8} (\kms{52\,026})
and a transmission \percent{\sim100},
we found that the contribution from the \CO{3}{2} line
to this filter is (\percent{\sim7.6}).
%
%
%
\subsection{Synchrotron emission \label{sec:synchrotron}}
%
Unlike the free-free emission coming from the \HII\ regions,
the modeling applied in this work does not take into account the contribution
of the synchrotron emission.
%
For this reason, the fluxes measured with \PLANCK{} need to be decontaminated
from this component.
%
Following the analysis of \citet[][]{2007A&A...475..133T}
we extrapolated the synchrotron emission from \cm{3.6} to the \PLANCK{}
filters assuming a non-thermal spectral index of 0.72
(see \Sec{Data:EFFELSBERG}).
%
We found non-thermal contributions of \percent{30} and \percent{5}
respectively for the \CAMERAmm{PLANCK}{10} and \mm{3.0} bands,
while for the other bands this contribution was found to be negligible.
%
%
%
\subsection{Error handling \label{sec:error}}
%
In our error analysis we took two types of error into account:
i) calibration, $\Delta_{\rm cal}$, \comment{using the values presented in \Tab{tab:observations}}, and
ii) measurement error due to background fluctuations, $\Delta_{\rm back}$.
%

%
The error due to the background fluctuations was calculated by assuming that
each pixel within the aperture has an error given by the standard deviation
of the background noise, $\sigma_{\rm back}$.
%
In addition, we have to take the error of the background into account
which was subtracted within an aperture of $N_{\rm apert}$ pixels.
%
This error is  $\sigma_{\rm back} N_{\rm apert} /\sqrt{N_{\rm back}}$, where
$N_{\rm back}$ is the number of pixels used to compute the level of background.
%
This gives \citep[see also][]{2012ApJ...745...95D} a total error
for the background subtracted flux of
%
\begin{equation}
  \Delta_{\rm back} =  \sigma_{\rm back}  \sqrt{N_{\rm apert} + \frac{N_{\rm apert}^2}{N_{\rm back}} }.
\end{equation}
%
The final error for the flux is the quadratic sum of
$\Delta_{\rm cal}$ and $\Delta_{\rm back}$.
%
In the case of the \PLANCK{} data, $\Delta_{\rm back}$ also includes
the error due to the CMB subtraction.
%
%
%


==> 97_IDL/SEDsexT100/TABLES/M33_Numbers.tex <==
%
% File generated with sed_phot2tex.pro on Wed Jan 27 18:38:48 2016
%
%
% GENERAL
%
\newcommand{\Distance}{0.840}
\newcommand{\ScaleLength}{2513}
\newcommand{\Inclination}{57}
%
%
% HII+PDR
%
\newcommand{\HIIperc}{32.3}
%
\newcommand{\METave}{0.2}
\newcommand{\METmin}{0.2}
\newcommand{\METmax}{0.4}
%
\newcommand{\AGEave}{4.0}
\newcommand{\AGEmin}{3.5}
\newcommand{\AGEmax}{4.0}
%
\newcommand{\CMPave}{4.0}
\newcommand{\CMPmin}{4.0}
\newcommand{\CMPmax}{4.5}
%
\newcommand{\PRSave}{8}
\newcommand{\PRSmin}{7}
\newcommand{\PRSmax}{8}
%
\newcommand{\COVave}{0.32}
\newcommand{\COVmin}{0.22}
\newcommand{\COVmax}{0.68}
%
\newcommand{\CHIaveHII}{3.59}
\newcommand{\CHIminHII}{0.77}
\newcommand{\CHImaxHII}{9.92}
%
\newcommand{\MCLave}{1.5}
\newcommand{\MCLmin}{0.2}
\newcommand{\MCLmax}{1.8}
%
\newcommand{\MCDave}{2.0}
\newcommand{\MCDmin}{1.6}
\newcommand{\MCDmax}{2.2}
%
\newcommand{\LUMaveHII}{0.31}
\newcommand{\LUMminHII}{0.26}
\newcommand{\LUMmaxHII}{0.37}
%
%
% DIFFUSE
%
\newcommand{\TAUave}{2.2}
\newcommand{\TAUmin}{1.8}
\newcommand{\TAUmax}{2.6}
%
\newcommand{\SFRave}{0.29}
\newcommand{\SFRmin}{0.25}
\newcommand{\SFRmax}{0.34}
%
\newcommand{\OLDave}{0.05}
\newcommand{\OLDmin}{0.05}
\newcommand{\OLDmax}{0.05}
%
\newcommand{\BDave}{0.0}
\newcommand{\BDmin}{0.0}
\newcommand{\BDmax}{0.0}
%
\newcommand{\CHIaveDIFF}{1.96}
\newcommand{\CHIminDIFF}{0.12}
\newcommand{\CHImaxDIFF}{5.03}
%
\newcommand{\MDDave}{13.8}
\newcommand{\MDDmin}{11.3}
\newcommand{\MDDmax}{16.3}
%
\newcommand{\LUMaveDIFF}{1.43}
\newcommand{\LUMminDIFF}{1.27}
\newcommand{\LUMmaxDIFF}{1.71}
%
%
% TOTAL
%
\newcommand{\LUMaveTOTAL}{1.74}
\newcommand{\LUMminTOTAL}{1.53}
\newcommand{\LUMmaxTOTAL}{2.08}
%
\newcommand{\MTDave}{15.7}
\newcommand{\MTDmin}{12.9}
\newcommand{\MTDmax}{18.5}
%
\newcommand{\ESCaveYOUNG}{57}
\newcommand{\ESCminYOUNG}{44}
\newcommand{\ESCmaxYOUNG}{78}
%
\newcommand{\ESCaveOLD}{7}
\newcommand{\ESCminOLD}{7}
\newcommand{\ESCmaxOLD}{7}
%
\newcommand{\SFRaveTotal}{0.43}
\newcommand{\SFRminTotal}{0.31}
\newcommand{\SFRmaxTotal}{1.07}
%
\newcommand{\GTDave}{108}
\newcommand{\GTDmin}{91}
\newcommand{\GTDmax}{132}
%
%
%


==> 97_IDL/SEDsexT100/TABLES/M33_Photometry.tex <==
%
%Table generated with sed_phot2tex.pro on Wed Jan 27 18:38:48 2016
%
\begin{tabular}{l c c c c c} \hline \noalign{\medskip}
\textbf{BAND} & $S^{\rm obs}_{\rm TOT}\rm\,(Jy)$ & $S^{\rm obs}_{\rm SF}\rm\,(Jy)$ & $S^{\rm obs}_{\rm DIFF}\rm\,(Jy)$ & $S^{\rm obs}_{\rm SF} / S^{\rm obs}_{\rm TOT}\rm\,(\%)$ \\\noalign{\smallskip} \hline \noalign{\medskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FUV             &  2.40        $\pm$0.27          &                -                &               -                &       -      \\\noalign{\medskip} 
NUV             &  3.52        $\pm$0.39          &                -                &               -                &       -      \\\noalign{\medskip} 
SLOANu          &  5.93        $\pm$0.32          &                -                &               -                &       -      \\\noalign{\medskip} 
Halpha          &  0.09        $\pm$0.02          &  0.03        $\pm$0.006         &                -                & 32.3         \\\noalign{\medskip} 
IRAC3           &  23.7        $\pm$1.26          &                -                &               -                &       -      \\\noalign{\medskip} 
IRAC4           &  15.3        $\pm$0.82          &                -                &               -                &       -      \\\noalign{\medskip} 
MIPS24          &  47.6        $\pm$3.05          &  15.9        $\pm$1.02          &  33.0        $\pm$2.68          &  33.4         \\\noalign{\medskip} 
PACS70          &  578         $\pm$64.7          &  176         $\pm$19.7          &  396         $\pm$48.5          &  30.5         \\\noalign{\medskip} 
PACS100         &  1387        $\pm$155           &  272         $\pm$30.4          &  1114        $\pm$136           &  19.6         \\\noalign{\medskip} 
PACS160         &  2162        $\pm$445           &  272         $\pm$56.2          &  1882        $\pm$399           &  12.6         \\\noalign{\medskip} 
SPIRE250        &  1316        $\pm$86.8          &  132         $\pm$8.75          &  1176        $\pm$97.3          &  10.1         \\\noalign{\medskip} 
PLANCK857GHz    &  777         $\pm$89.5          &                -                & 715         $\pm$82.3          &  8.0          \\\noalign{\medskip} 
SPIRE350        &  718         $\pm$47.4          &  59.3        $\pm$3.91          &  663         $\pm$54.9          &  8.3          \\\noalign{\medskip} 
SPIRE500        &  319         $\pm$21.0          &  24.0        $\pm$1.58          &  293         $\pm$24.3          &  7.5          \\\noalign{\medskip} 
PLANCK545GHz    &  305         $\pm$35.1          &                -                & 288         $\pm$33.2          &  5.5          \\\noalign{\medskip} 
PLANCK353GHz    &  91.9        $\pm$6.91          &                -                & 87.7        $\pm$6.60          &  4.6          \\\noalign{\medskip} 
LABOCA870       &                -                & 6.67        $\pm$0.75          &                -                &       -      \\\noalign{\medskip} 
PLANCK217GHz    &  21.7        $\pm$1.95          &                -                & 20.6        $\pm$1.86          &  4.7          \\\noalign{\medskip} 
PLANCK143GHz    &  4.27        $\pm$0.57          &                -                & 3.77        $\pm$0.51          &  11.7         \\\noalign{\medskip} 
PLANCK100GHz    &  1.86        $\pm$0.19          &                -                & 1.46        $\pm$0.15          &  21.5         \\\noalign{\medskip} 
PLANCK30GHz     &  0.40        $\pm$0.09          &                -                &               -                &       -      \\\noalign{\medskip} 
EFFELS8GHz      &  0.44        $\pm$0.05          &  0.44        $\pm$0.05          &                -                & 100.0        \\\noalign{\medskip} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \\
\end{tabular}


==> 97_IDL/SEDsexT100/TABLES/M33_RatioObsModel.tex <==
%
%Table generated with sed_phot2tex.pro on Wed Jan 27 18:38:48 2016
%
\begin{tabular}{l c c c c c c} \hline \noalign{\medskip}
\textbf{BAND} & $ \frac{ S^{\rm obs}_{\rm SF} } { S^{\rm mod}_{\rm SF} } $ & $ \frac{ \Delta_{\rm SF} } { \sqrt{ \left( \delta^{\rm obs}_{\rm SF} \right)^2 + \left( \delta^{\rm mod}_{\rm SF} \right)^2} } $ & $ \frac{ S^{\rm obs}_{\rm DIFF} } { S^{\rm mod}_{\rm DIFF} } $ & $ \frac{ \Delta_{\rm DIFF} } { \sqrt{ \left( \delta^{\rm obs}_{\rm DIFF} \right)^2 + \left( \delta^{\rm mod}_{\rm DIFF} \right)^2} } $ & $ \frac{ S^{\rm obs}_{\rm TOT} } { S^{\rm mod}_{\rm TOT} } $ & $ \frac{ \Delta_{\rm TOT} } { \sqrt{ \left( \delta^{\rm obs}_{\rm TOT} \right)^2 + \left( \delta^{\rm mod}_{\rm TOT} \right)^2} } $ \\ \noalign{\smallskip} \hline \noalign{\medskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FUV            &             -           &   -   &             -           &   -   & \Vlim{1.67}{2.40}{18.16} & 3.08  \\\noalign{\medskip}
NUV            &             -           &   -   &             -           &   -   & \Vlim{2.13}{2.78}{5.75} & 5.50  \\\noalign{\medskip}
SLOANu         &             -           &   -   &             -           &   -   & \Vlim{1.10}{1.33}{1.83} & 1.53  \\\noalign{\medskip}
Halpha         &             -           &   -   &             -           &   -   & \Vlim{0.00}{0.00}{0.00} & -4.11 \\\noalign{\medskip}
IRAC3          &             -           &   -   &             -           &   -   & \Vlim{0.97}{0.98}{0.99} & -0.29 \\\noalign{\medskip}
IRAC4          &             -           &   -   &             -           &   -   & \Vlim{1.13}{1.14}{1.16} & 2.62  \\\noalign{\medskip}
MIPS24         & \Vlim{0.92}{1.05}{1.27} & 0.34  & \Vlim{0.84}{1.04}{1.18} & 0.16  & \Vlim{0.84}{1.02}{1.18} & 0.10  \\\noalign{\medskip}
PACS70         & \Vlim{0.85}{1.03}{1.19} & 0.11  & \Vlim{0.83}{1.08}{1.25} & 0.25  & \Vlim{0.84}{1.08}{1.25} & 0.43  \\\noalign{\medskip}
PACS100        & \Vlim{0.87}{1.08}{1.32} & 0.29  & \Vlim{0.78}{0.96}{1.09} & -0.26 & \Vlim{0.79}{0.98}{1.13} & -0.13 \\\noalign{\medskip}
PACS160        & \Vlim{0.90}{1.07}{1.33} & 0.26  & \Vlim{0.84}{0.95}{1.06} & -0.22 & \Vlim{0.85}{0.96}{1.09} & -0.15 \\\noalign{\medskip}
SPIRE250       & \Vlim{0.87}{1.00}{1.23} & -0.01 & \Vlim{0.78}{0.87}{0.97} & -0.98 & \Vlim{0.80}{0.89}{1.00} & -0.88 \\\noalign{\medskip}
PLANCK857GHz   &             -           &   -   & \Vlim{0.89}{0.99}{1.12} & -0.05 & \Vlim{0.89}{0.99}{1.13} & -0.05 \\\noalign{\medskip}
SPIRE350       & \Vlim{0.93}{1.06}{1.31} & 0.40  & \Vlim{0.91}{1.01}{1.14} & 0.07  & \Vlim{0.91}{1.01}{1.15} & 0.05  \\\noalign{\medskip}
SPIRE500       & \Vlim{1.04}{1.20}{1.47} & 1.22  & \Vlim{1.00}{1.13}{1.29} & 0.84  & \Vlim{1.01}{1.14}{1.31} & 0.97  \\\noalign{\medskip}
PLANCK545GHz   &             -           &   -   & \Vlim{1.15}{1.29}{1.49} & 1.72  & \Vlim{1.13}{1.27}{1.47} & 1.59  \\\noalign{\medskip}
PLANCK353GHz   &             -           &   -   & \Vlim{1.35}{1.54}{1.79} & 3.39  & \Vlim{1.32}{1.50}{1.75} & 3.15  \\\noalign{\medskip}
LABOCA870      & \Vlim{1.50}{1.71}{2.07} & 3.89  &             -           &   -   &             -           &   -   \\\noalign{\medskip}
PLANCK217GHz   &             -           &   -   & \Vlim{1.73}{1.99}{2.33} & 5.70  & \Vlim{1.66}{1.90}{2.23} & 5.27  \\\noalign{\medskip}
PLANCK143GHz   &             -           &   -   & \Vlim{1.65}{1.90}{2.24} & 4.44  & \Vlim{1.51}{1.74}{2.06} & 3.64  \\\noalign{\medskip}
PLANCK100GHz   &             -           &   -   & \Vlim{2.45}{2.83}{3.32} & 9.87  & \Vlim{1.75}{2.04}{2.48} & 5.40  \\\noalign{\medskip}
PLANCK30GHz    &             -           &   -   &             -           &   -   & \Vlim{0.79}{0.94}{1.19} & -0.21 \\\noalign{\medskip}
EFFELS8GHz     & \Vlim{0.74}{0.88}{1.12} & -0.49 &             -           &   -   & \Vlim{0.74}{0.88}{1.12} & -0.49 \\\noalign{\medskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \\
\end{tabular}


==> 97_IDL/SEDsexT20/TABLES/M33_Numbers.tex <==
%
% File generated with sed_phot2tex.pro on Wed Jan 27 18:21:36 2016
%
%
% GENERAL
%
\newcommand{\Distance}{0.840}
\newcommand{\ScaleLength}{2513}
\newcommand{\Inclination}{57}
%
%
% HII+PDR
%
\newcommand{\HIIperc}{45.9}
%
\newcommand{\METave}{0.2}
\newcommand{\METmin}{0.2}
\newcommand{\METmax}{0.2}
%
\newcommand{\AGEave}{4.0}
\newcommand{\AGEmin}{3.5}
\newcommand{\AGEmax}{4.0}
%
\newcommand{\CMPave}{4.0}
\newcommand{\CMPmin}{4.0}
\newcommand{\CMPmax}{4.0}
%
\newcommand{\PRSave}{8}
\newcommand{\PRSmin}{8}
\newcommand{\PRSmax}{8}
%
\newcommand{\COVave}{0.54}
\newcommand{\COVmin}{0.42}
\newcommand{\COVmax}{0.74}
%
\newcommand{\CHIaveHII}{5.95}
\newcommand{\CHIminHII}{2.42}
\newcommand{\CHImaxHII}{14.16}
%
\newcommand{\MCLave}{1.6}
\newcommand{\MCLmin}{1.0}
\newcommand{\MCLmax}{1.9}
%
\newcommand{\MCDave}{3.5}
\newcommand{\MCDmin}{3.0}
\newcommand{\MCDmax}{4.0}
%
\newcommand{\LUMaveHII}{0.47}
\newcommand{\LUMminHII}{0.41}
\newcommand{\LUMmaxHII}{0.53}
%
%
% DIFFUSE
%
\newcommand{\TAUave}{2.0}
\newcommand{\TAUmin}{1.6}
\newcommand{\TAUmax}{2.6}
%
\newcommand{\SFRave}{0.25}
\newcommand{\SFRmin}{0.20}
\newcommand{\SFRmax}{0.29}
%
\newcommand{\OLDave}{0.05}
\newcommand{\OLDmin}{0.05}
\newcommand{\OLDmax}{0.05}
%
\newcommand{\BDave}{0.0}
\newcommand{\BDmin}{0.0}
\newcommand{\BDmax}{0.0}
%
\newcommand{\CHIaveDIFF}{1.75}
\newcommand{\CHIminDIFF}{0.31}
\newcommand{\CHImaxDIFF}{4.70}
%
\newcommand{\MDDave}{12.5}
\newcommand{\MDDmin}{10.0}
\newcommand{\MDDmax}{16.3}
%
\newcommand{\LUMaveDIFF}{1.25}
\newcommand{\LUMminDIFF}{1.08}
\newcommand{\LUMmaxDIFF}{1.49}
%
%
% TOTAL
%
\newcommand{\LUMaveTOTAL}{1.72}
\newcommand{\LUMminTOTAL}{1.49}
\newcommand{\LUMmaxTOTAL}{2.02}
%
\newcommand{\MTDave}{16.0}
\newcommand{\MTDmin}{13.0}
\newcommand{\MTDmax}{20.3}
%
\newcommand{\ESCaveYOUNG}{72}
\newcommand{\ESCminYOUNG}{60}
\newcommand{\ESCmaxYOUNG}{84}
%
\newcommand{\ESCaveOLD}{7}
\newcommand{\ESCminOLD}{7}
\newcommand{\ESCmaxOLD}{7}
%
\newcommand{\SFRaveTotal}{0.53}
\newcommand{\SFRminTotal}{0.34}
\newcommand{\SFRmaxTotal}{1.13}
%
\newcommand{\GTDave}{106}
\newcommand{\GTDmin}{83}
\newcommand{\GTDmax}{130}
%
%
%


==> 97_IDL/SEDsexT20/TABLES/M33_Photometry.tex <==
%
%Table generated with sed_phot2tex.pro on Wed Jan 27 18:21:36 2016
%
\begin{tabular}{l c c c c c} \hline \noalign{\medskip}
\textbf{BAND} & $S^{\rm obs}_{\rm TOT}\rm\,(Jy)$ & $S^{\rm obs}_{\rm SF}\rm\,(Jy)$ & $S^{\rm obs}_{\rm DIFF}\rm\,(Jy)$ & $S^{\rm obs}_{\rm SF} / S^{\rm obs}_{\rm TOT}\rm\,(\%)$ \\\noalign{\smallskip} \hline \noalign{\medskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\GALEX{FUV}               &  2.40        $\pm$0.27          &                -                &               -                &       -      \\\noalign{\medskip}
\GALEX{NUV}               &  3.52        $\pm$0.39          &                -                &               -                &       -      \\\noalign{\medskip}
\SLOAN{u}                 &  5.93        $\pm$0.32          &                -                &               -                &       -      \\\noalign{\medskip}
\Halpha                   &  0.09        $\pm$0.02          &  0.04        $\pm$0.008         &                -                & 45.9         \\\noalign{\medskip}
\CAMERAmu{IRAC}{3.6}      &  23.7        $\pm$1.26          &                -                &               -                &       -      \\\noalign{\medskip}
\CAMERAmu{IRAC}{4.5}      &  15.3        $\pm$0.82          &                -                &               -                &       -      \\\noalign{\medskip}
\CAMERAmu{MIPS}{24}       &  47.6        $\pm$3.05          &  21.0        $\pm$1.34          &  27.7        $\pm$2.25          &  44.1         \\\noalign{\medskip}
\CAMERAmu{PACS}{70}       &  578         $\pm$64.7          &  243         $\pm$27.2          &  330         $\pm$40.4          &  42.1         \\\noalign{\medskip}
\CAMERAmu{PACS}{100}      &  1387        $\pm$155           &  400         $\pm$44.7          &  986         $\pm$120           &  28.8         \\\noalign{\medskip}
\CAMERAmu{PACS}{160}      &  2162        $\pm$445           &  439         $\pm$90.5          &  1716        $\pm$364           &  20.3         \\\noalign{\medskip}
\CAMERAmu{SPIRE}{250}     &  1316        $\pm$86.8          &  237         $\pm$15.7          &  1072        $\pm$88.7          &  18.0         \\\noalign{\medskip}
\CAMERAmu{PLANCK}{350}    &  777         $\pm$89.5          &                -                & 665         $\pm$76.7          &  14.3         \\\noalign{\medskip}
\CAMERAmu{SPIRE}{350}     &  718         $\pm$47.4          &  110         $\pm$7.29          &  611         $\pm$50.6          &  15.4         \\\noalign{\medskip}
\CAMERAmu{SPIRE}{500}     &  319         $\pm$21.0          &  46.6        $\pm$3.07          &  270         $\pm$22.4          &  14.6         \\\noalign{\medskip}
\CAMERAmu{PLANCK}{550}    &  305         $\pm$35.1          &                -                & 274         $\pm$31.6          &  10.0         \\\noalign{\medskip}
\CAMERAmu{PLANCK}{850}    &  91.9        $\pm$6.91          &                -                & 84.5        $\pm$6.35          &  8.1          \\\noalign{\medskip}
\CAMERAmu{LABOCA}{870}    &                -                & 12.4        $\pm$1.38          &                -                &       -      \\\noalign{\medskip}
\CAMERAmm{PLANCK}{1.4}    &  21.7        $\pm$1.95          &                -                & 20.0        $\pm$1.81          &  7.5          \\\noalign{\medskip}
\CAMERAmm{PLANCK}{2.1}    &  4.27        $\pm$0.57          &                -                & 3.60        $\pm$0.48          &  15.5         \\\noalign{\medskip}
\CAMERAmm{PLANCK}{3.0}    &  1.86        $\pm$0.19          &                -                & 1.39        $\pm$0.14          &  25.3         \\\noalign{\medskip}
\CAMERAmm{PLANCK}{10}     &  0.40        $\pm$0.09          &                -                &               -                &       -      \\\noalign{\medskip}
\CAMERAmm{S}{36}          &  0.44        $\pm$0.05          &  0.44        $\pm$0.05          &                -                & 100.0        \\\noalign{\medskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \\
\end{tabular}


==> 97_IDL/SEDsexT60/TABLES/M33_Numbers.tex <==
%
% File generated with sed_phot2tex.pro on Wed Jan 27 18:31:17 2016
%
%
% GENERAL
%
\newcommand{\Distance}{0.840}
\newcommand{\ScaleLength}{2513}
\newcommand{\Inclination}{57}
%
%
% HII+PDR
%
\newcommand{\HIIperc}{37.7}
%
\newcommand{\METave}{0.2}
\newcommand{\METmin}{0.2}
\newcommand{\METmax}{0.2}
%
\newcommand{\AGEave}{4.0}
\newcommand{\AGEmin}{3.5}
\newcommand{\AGEmax}{4.0}
%
\newcommand{\CMPave}{4.0}
\newcommand{\CMPmin}{4.0}
\newcommand{\CMPmax}{4.0}
%
\newcommand{\PRSave}{8}
\newcommand{\PRSmin}{8}
\newcommand{\PRSmax}{8}
%
\newcommand{\COVave}{0.40}
\newcommand{\COVmin}{0.32}
\newcommand{\COVmax}{0.74}
%
\newcommand{\CHIaveHII}{4.29}
\newcommand{\CHIminHII}{0.82}
\newcommand{\CHImaxHII}{9.97}
%
\newcommand{\MCLave}{1.6}
\newcommand{\MCLmin}{0.8}
\newcommand{\MCLmax}{1.9}
%
\newcommand{\MCDave}{2.5}
\newcommand{\MCDmin}{2.2}
\newcommand{\MCDmax}{2.9}
%
\newcommand{\LUMaveHII}{0.37}
\newcommand{\LUMminHII}{0.33}
\newcommand{\LUMmaxHII}{0.43}
%
%
% DIFFUSE
%
\newcommand{\TAUave}{2.2}
\newcommand{\TAUmin}{1.6}
\newcommand{\TAUmax}{2.6}
%
\newcommand{\SFRave}{0.25}
\newcommand{\SFRmin}{0.20}
\newcommand{\SFRmax}{0.29}
%
\newcommand{\OLDave}{0.05}
\newcommand{\OLDmin}{0.05}
\newcommand{\OLDmax}{0.05}
%
\newcommand{\BDave}{0.0}
\newcommand{\BDmin}{0.0}
\newcommand{\BDmax}{0.0}
%
\newcommand{\CHIaveDIFF}{1.73}
\newcommand{\CHIminDIFF}{0.29}
\newcommand{\CHImaxDIFF}{4.64}
%
\newcommand{\MDDave}{13.8}
\newcommand{\MDDmin}{10.0}
\newcommand{\MDDmax}{16.3}
%
\newcommand{\LUMaveDIFF}{1.35}
\newcommand{\LUMminDIFF}{1.11}
\newcommand{\LUMmaxDIFF}{1.54}
%
%
% TOTAL
%
\newcommand{\LUMaveTOTAL}{1.73}
\newcommand{\LUMminTOTAL}{1.44}
\newcommand{\LUMmaxTOTAL}{1.97}
%
\newcommand{\MTDave}{16.3}
\newcommand{\MTDmin}{12.2}
\newcommand{\MTDmax}{19.2}
%
\newcommand{\ESCaveYOUNG}{67}
\newcommand{\ESCminYOUNG}{57}
\newcommand{\ESCmaxYOUNG}{84}
%
\newcommand{\ESCaveOLD}{7}
\newcommand{\ESCminOLD}{7}
\newcommand{\ESCmaxOLD}{7}
%
\newcommand{\SFRaveTotal}{0.41}
\newcommand{\SFRminTotal}{0.29}
\newcommand{\SFRmaxTotal}{1.13}
%
\newcommand{\GTDave}{104}
\newcommand{\GTDmin}{88}
\newcommand{\GTDmax}{139}
%
%
%


==> 97_IDL/SEDsexT60/TABLES/M33_Photometry.tex <==
%
%Table generated with sed_phot2tex.pro on Wed Jan 27 18:31:17 2016
%
\begin{tabular}{l c c c c c} \hline \noalign{\medskip}
\textbf{BAND} & $S^{\rm obs}_{\rm TOT}\rm\,(Jy)$ & $S^{\rm obs}_{\rm SF}\rm\,(Jy)$ & $S^{\rm obs}_{\rm DIFF}\rm\,(Jy)$ & $S^{\rm obs}_{\rm SF} / S^{\rm obs}_{\rm TOT}\rm\,(\%)$ \\\noalign{\smallskip} \hline \noalign{\medskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\GALEX{FUV}               &  2.40        $\pm$0.27          &                -                &               -                &       -      \\\noalign{\medskip}
\GALEX{NUV}               &  3.52        $\pm$0.39          &                -                &               -                &       -      \\\noalign{\medskip}
\SLOAN{u}                 &  5.93        $\pm$0.32          &                -                &               -                &       -      \\\noalign{\medskip}
\Halpha                   &  0.09        $\pm$0.02          &  0.03        $\pm$0.007         &                -                & 37.7         \\\noalign{\medskip}
\CAMERAmu{IRAC}{3.6}      &  23.7        $\pm$1.26          &                -                &               -                &       -      \\\noalign{\medskip}
\CAMERAmu{IRAC}{4.5}      &  15.3        $\pm$0.82          &                -                &               -                &       -      \\\noalign{\medskip}
\CAMERAmu{MIPS}{24}       &  47.6        $\pm$3.05          &  18.2        $\pm$1.17          &  30.6        $\pm$2.48          &  38.3         \\\noalign{\medskip}
\CAMERAmu{PACS}{70}       &  578         $\pm$64.7          &  205         $\pm$23.0          &  367         $\pm$45.0          &  35.5         \\\noalign{\medskip}
\CAMERAmu{PACS}{100}      &  1387        $\pm$155           &  324         $\pm$36.3          &  1062        $\pm$130           &  23.4         \\\noalign{\medskip}
\CAMERAmu{PACS}{160}      &  2162        $\pm$445           &  335         $\pm$69.2          &  1819        $\pm$385           &  15.5         \\\noalign{\medskip}
\CAMERAmu{SPIRE}{250}     &  1316        $\pm$86.8          &  168         $\pm$11.1          &  1140        $\pm$94.4          &  12.8         \\\noalign{\medskip}
\CAMERAmu{PLANCK}{350}    &  777         $\pm$89.5          &                -                & 697         $\pm$80.3          &  10.2         \\\noalign{\medskip}
\CAMERAmu{SPIRE}{350}     &  718         $\pm$47.4          &  76.0        $\pm$5.01          &  646         $\pm$53.5          &  10.6         \\\noalign{\medskip}
\CAMERAmu{SPIRE}{500}     &  319         $\pm$21.0          &  31.1        $\pm$2.05          &  286         $\pm$23.7          &  9.7          \\\noalign{\medskip}
\CAMERAmu{PLANCK}{550}    &  305         $\pm$35.1          &                -                & 283         $\pm$32.6          &  7.1          \\\noalign{\medskip}
\CAMERAmu{PLANCK}{850}    &  91.9        $\pm$6.91          &                -                & 86.6        $\pm$6.51          &  5.8          \\\noalign{\medskip}
\CAMERAmu{LABOCA}{870}    &                -                & 8.47        $\pm$0.95          &                -                &       -      \\\noalign{\medskip}
\CAMERAmm{PLANCK}{1.4}    &  21.7        $\pm$1.95          &                -                & 20.4        $\pm$1.84          &  5.7          \\\noalign{\medskip}
\CAMERAmm{PLANCK}{2.1}    &  4.27        $\pm$0.57          &                -                & 3.71        $\pm$0.50          &  13.1         \\\noalign{\medskip}
\CAMERAmm{PLANCK}{3.0}    &  1.86        $\pm$0.19          &                -                & 1.43        $\pm$0.14          &  23.0         \\\noalign{\medskip}
\CAMERAmm{PLANCK}{10}     &  0.40        $\pm$0.09          &                -                &               -                &       -      \\\noalign{\medskip}
\CAMERAmm{S}{36}          &  0.44        $\pm$0.05          &  0.44        $\pm$0.05          &                -                & 100.0        \\\noalign{\medskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \\
\end{tabular}


==> 97_IDL/SEDsexT80/TABLES/M33_Numbers.tex <==
%
% File generated with sed_phot2tex.pro on Wed Jan 27 18:35:20 2016
%
%
% GENERAL
%
\newcommand{\Distance}{0.840}
\newcommand{\ScaleLength}{2513}
\newcommand{\Inclination}{57}
%
%
% HII+PDR
%
\newcommand{\HIIperc}{34.6}
%
\newcommand{\METave}{0.2}
\newcommand{\METmin}{0.2}
\newcommand{\METmax}{0.4}
%
\newcommand{\AGEave}{4.0}
\newcommand{\AGEmin}{3.5}
\newcommand{\AGEmax}{4.0}
%
\newcommand{\CMPave}{4.0}
\newcommand{\CMPmin}{4.0}
\newcommand{\CMPmax}{4.5}
%
\newcommand{\PRSave}{8}
\newcommand{\PRSmin}{8}
\newcommand{\PRSmax}{8}
%
\newcommand{\COVave}{0.34}
\newcommand{\COVmin}{0.22}
\newcommand{\COVmax}{0.72}
%
\newcommand{\CHIaveHII}{4.42}
\newcommand{\CHIminHII}{1.27}
\newcommand{\CHImaxHII}{9.44}
%
\newcommand{\MCLave}{1.6}
\newcommand{\MCLmin}{0.3}
\newcommand{\MCLmax}{1.8}
%
\newcommand{\MCDave}{2.2}
\newcommand{\MCDmin}{1.9}
\newcommand{\MCDmax}{2.5}
%
\newcommand{\LUMaveHII}{0.34}
\newcommand{\LUMminHII}{0.30}
\newcommand{\LUMmaxHII}{0.39}
%
%
% DIFFUSE
%
\newcommand{\TAUave}{2.2}
\newcommand{\TAUmin}{1.6}
\newcommand{\TAUmax}{2.6}
%
\newcommand{\SFRave}{0.25}
\newcommand{\SFRmin}{0.25}
\newcommand{\SFRmax}{0.34}
%
\newcommand{\OLDave}{0.05}
\newcommand{\OLDmin}{0.05}
\newcommand{\OLDmax}{0.05}
%
\newcommand{\BDave}{0.0}
\newcommand{\BDmin}{0.0}
\newcommand{\BDmax}{0.0}
%
\newcommand{\CHIaveDIFF}{1.94}
\newcommand{\CHIminDIFF}{0.46}
\newcommand{\CHImaxDIFF}{4.58}
%
\newcommand{\MDDave}{13.8}
\newcommand{\MDDmin}{10.0}
\newcommand{\MDDmax}{16.3}
%
\newcommand{\LUMaveDIFF}{1.39}
\newcommand{\LUMminDIFF}{1.24}
\newcommand{\LUMmaxDIFF}{1.56}
%
%
% TOTAL
%
\newcommand{\LUMaveTOTAL}{1.73}
\newcommand{\LUMminTOTAL}{1.53}
\newcommand{\LUMmaxTOTAL}{1.96}
%
\newcommand{\MTDave}{16.0}
\newcommand{\MTDmin}{12.0}
\newcommand{\MTDmax}{18.8}
%
\newcommand{\ESCaveYOUNG}{65}
\newcommand{\ESCminYOUNG}{44}
\newcommand{\ESCmaxYOUNG}{80}
%
\newcommand{\ESCaveOLD}{7}
\newcommand{\ESCminOLD}{7}
\newcommand{\ESCmaxOLD}{7}
%
\newcommand{\SFRaveTotal}{0.37}
\newcommand{\SFRminTotal}{0.31}
\newcommand{\SFRmaxTotal}{1.23}
%
\newcommand{\GTDave}{106}
\newcommand{\GTDmin}{90}
\newcommand{\GTDmax}{142}
%
%
%


==> 97_IDL/SEDsexT80/TABLES/M33_Photometry.tex <==
%
%Table generated with sed_phot2tex.pro on Wed Jan 27 18:35:20 2016
%
\begin{tabular}{l c c c c c} \hline \noalign{\medskip}
\textbf{BAND} & $S^{\rm obs}_{\rm TOT}\rm\,(Jy)$ & $S^{\rm obs}_{\rm SF}\rm\,(Jy)$ & $S^{\rm obs}_{\rm DIFF}\rm\,(Jy)$ & $S^{\rm obs}_{\rm SF} / S^{\rm obs}_{\rm TOT}\rm\,(\%)$ \\\noalign{\smallskip} \hline \noalign{\medskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FUV             &  2.40        $\pm$0.27          &                -                &               -                &       -      \\\noalign{\medskip} 
NUV             &  3.52        $\pm$0.39          &                -                &               -                &       -      \\\noalign{\medskip} 
SLOANu          &  5.93        $\pm$0.32          &                -                &               -                &       -      \\\noalign{\medskip} 
Halpha          &  0.09        $\pm$0.02          &  0.03        $\pm$0.006         &                -                & 34.6         \\\noalign{\medskip} 
IRAC3           &  23.7        $\pm$1.26          &                -                &               -                &       -      \\\noalign{\medskip} 
IRAC4           &  15.3        $\pm$0.82          &                -                &               -                &       -      \\\noalign{\medskip} 
MIPS24          &  47.6        $\pm$3.05          &  17.3        $\pm$1.11          &  31.5        $\pm$2.56          &  36.4         \\\noalign{\medskip} 
PACS70          &  578         $\pm$64.7          &  191         $\pm$21.4          &  381         $\pm$46.7          &  33.1         \\\noalign{\medskip} 
PACS100         &  1387        $\pm$155           &  298         $\pm$33.4          &  1088        $\pm$133           &  21.6         \\\noalign{\medskip} 
PACS160         &  2162        $\pm$445           &  302         $\pm$62.4          &  1852        $\pm$392           &  14.0         \\\noalign{\medskip} 
SPIRE250        &  1316        $\pm$86.8          &  148         $\pm$9.80          &  1160        $\pm$96.0          &  11.3         \\\noalign{\medskip} 
PLANCK857GHz    &  777         $\pm$89.5          &                -                & 708         $\pm$81.5          &  8.9          \\\noalign{\medskip} 
SPIRE350        &  718         $\pm$47.4          &  66.6        $\pm$4.39          &  656         $\pm$54.3          &  9.3          \\\noalign{\medskip} 
SPIRE500        &  319         $\pm$21.0          &  27.1        $\pm$1.79          &  290         $\pm$24.0          &  8.5          \\\noalign{\medskip} 
PLANCK545GHz    &  305         $\pm$35.1          &                -                & 286         $\pm$32.9          &  6.2          \\\noalign{\medskip} 
PLANCK353GHz    &  91.9        $\pm$6.91          &                -                & 87.2        $\pm$6.56          &  5.1          \\\noalign{\medskip} 
LABOCA870       &                -                & 7.49        $\pm$0.84          &                -                &       -      \\\noalign{\medskip} 
PLANCK217GHz    &  21.7        $\pm$1.95          &                -                & 20.6        $\pm$1.85          &  5.1          \\\noalign{\medskip} 
PLANCK143GHz    &  4.27        $\pm$0.57          &                -                & 3.74        $\pm$0.50          &  12.4         \\\noalign{\medskip} 
PLANCK100GHz    &  1.86        $\pm$0.19          &                -                & 1.44        $\pm$0.15          &  22.6         \\\noalign{\medskip} 
PLANCK30GHz     &  0.40        $\pm$0.09          &                -                &               -                &       -      \\\noalign{\medskip} 
EFFELS8GHz      &  0.44        $\pm$0.05          &  0.44        $\pm$0.05          &                -                & 100.0        \\\noalign{\medskip} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \\
\end{tabular}


==> 97_IDL/SEDsexT80/TABLES/M33_RatioObsModel.tex <==
%
%Table generated with sed_phot2tex.pro on Wed Jan 27 18:35:20 2016
%
\begin{tabular}{l c c c c c c} \hline \noalign{\medskip}
\textbf{BAND} & $ \frac{ S^{\rm obs}_{\rm SF} } { S^{\rm mod}_{\rm SF} } $ & $ \frac{ \Delta_{\rm SF} } { \sqrt{ \left( \delta^{\rm obs}_{\rm SF} \right)^2 + \left( \delta^{\rm mod}_{\rm SF} \right)^2} } $ & $ \frac{ S^{\rm obs}_{\rm DIFF} } { S^{\rm mod}_{\rm DIFF} } $ & $ \frac{ \Delta_{\rm DIFF} } { \sqrt{ \left( \delta^{\rm obs}_{\rm DIFF} \right)^2 + \left( \delta^{\rm mod}_{\rm DIFF} \right)^2} } $ & $ \frac{ S^{\rm obs}_{\rm TOT} } { S^{\rm mod}_{\rm TOT} } $ & $ \frac{ \Delta_{\rm TOT} } { \sqrt{ \left( \delta^{\rm obs}_{\rm TOT} \right)^2 + \left( \delta^{\rm mod}_{\rm TOT} \right)^2} } $ \\ \noalign{\smallskip} \hline \noalign{\medskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FUV            &             -           &   -   &             -           &   -   & \Vlim{1.67}{3.02}{44.31} & 2.46  \\\noalign{\medskip}
NUV            &             -           &   -   &             -           &   -   & \Vlim{2.13}{3.41}{6.26} & 3.94  \\\noalign{\medskip}
SLOANu         &             -           &   -   &             -           &   -   & \Vlim{1.10}{1.61}{1.86} & 1.31  \\\noalign{\medskip}
Halpha         &             -           &   -   &             -           &   -   & \Vlim{0.00}{0.00}{0.00} & -4.81 \\\noalign{\medskip}
IRAC3          &             -           &   -   &             -           &   -   & \Vlim{0.97}{0.99}{0.99} & -0.10 \\\noalign{\medskip}
IRAC4          &             -           &   -   &             -           &   -   & \Vlim{1.13}{1.15}{1.16} & 2.69  \\\noalign{\medskip}
MIPS24         & \Vlim{0.91}{1.06}{1.20} & 0.35  & \Vlim{0.91}{1.03}{1.13} & 0.19  & \Vlim{0.89}{1.01}{1.13} & 0.11  \\\noalign{\medskip}
PACS70         & \Vlim{0.88}{1.02}{1.15} & 0.09  & \Vlim{0.88}{1.09}{1.21} & 0.33  & \Vlim{0.89}{1.07}{1.20} & 0.49  \\\noalign{\medskip}
PACS100        & \Vlim{0.90}{1.06}{1.22} & 0.29  & \Vlim{0.86}{0.97}{1.06} & -0.21 & \Vlim{0.87}{0.99}{1.09} & -0.09 \\\noalign{\medskip}
PACS160        & \Vlim{0.93}{1.06}{1.21} & 0.25  & \Vlim{0.88}{0.96}{1.09} & -0.17 & \Vlim{0.89}{0.98}{1.11} & -0.10 \\\noalign{\medskip}
SPIRE250       & \Vlim{0.86}{1.00}{1.13} & 0.01  & \Vlim{0.80}{0.88}{1.05} & -0.65 & \Vlim{0.81}{0.90}{1.07} & -0.60 \\\noalign{\medskip}
PLANCK857GHz   &             -           &   -   & \Vlim{0.89}{1.00}{1.23} & 0.00  & \Vlim{0.89}{1.00}{1.22} & 0.00  \\\noalign{\medskip}
SPIRE350       & \Vlim{0.92}{1.07}{1.21} & 0.40  & \Vlim{0.90}{1.02}{1.25} & 0.11  & \Vlim{0.90}{1.01}{1.24} & 0.08  \\\noalign{\medskip}
SPIRE500       & \Vlim{1.04}{1.22}{1.41} & 1.16  & \Vlim{0.99}{1.13}{1.42} & 0.80  & \Vlim{1.00}{1.15}{1.43} & 0.91  \\\noalign{\medskip}
PLANCK545GHz   &             -           &   -   & \Vlim{1.14}{1.31}{1.65} & 1.66  & \Vlim{1.12}{1.28}{1.60} & 1.51  \\\noalign{\medskip}
PLANCK353GHz   &             -           &   -   & \Vlim{1.34}{1.55}{1.98} & 3.20  & \Vlim{1.30}{1.51}{1.92} & 2.93  \\\noalign{\medskip}
LABOCA870      & \Vlim{1.48}{1.74}{2.06} & 3.60  &             -           &   -   &             -           &   -   \\\noalign{\medskip}
PLANCK217GHz   &             -           &   -   & \Vlim{1.73}{2.01}{2.59} & 5.41  & \Vlim{1.64}{1.91}{2.45} & 4.94  \\\noalign{\medskip}
PLANCK143GHz   &             -           &   -   & \Vlim{1.64}{1.91}{2.48} & 4.25  & \Vlim{1.49}{1.73}{2.26} & 3.50  \\\noalign{\medskip}
PLANCK100GHz   &             -           &   -   & \Vlim{2.41}{2.82}{3.66} & 9.26  & \Vlim{1.73}{2.01}{2.68} & 5.32  \\\noalign{\medskip}
PLANCK30GHz    &             -           &   -   &             -           &   -   & \Vlim{0.77}{0.89}{1.24} & -0.29 \\\noalign{\medskip}
EFFELS8GHz     & \Vlim{0.73}{0.84}{1.17} & -0.52 &             -           &   -   & \Vlim{0.73}{0.84}{1.17} & -0.52 \\\noalign{\medskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \\
\end{tabular}

